A virtually connected probabilistic computer as a solver for higher-order, densely connected, or reconfigurable combinatorial optimisation problems

Recently, there has been growing interest in unconventional computing as an approach for solving NP-hard problems, by developing dedicated hardware to find solutions more efficiently than conventional CPUs. In many of these approaches, however, certain problem geometries must be transformed into forms that are more amenable to the available hardware topology through techniques such as embedding, sparsification, and quadratisation, leading to a deterioration in solution quality. A probabilistic computing architecture based on high speed photonic quantum random number generators was recently proposed which utilises virtual hardware connections (Aboushelbaya et al., 2025), circumventing the necessity for such procedures. Here, we discuss the applicability of virtually connected hardware for running heuristic solving methods to solve a selection of problems, which due to their geometry, would suffer from topological hardware restrictions. We also employ greedy graph colouring algorithms for hardware parallelisation, allowing favourable scaling for desirable solution qualities. To emphasise the difficulty in solving these problems on physically connected hardware, we demonstrate the increase in problem size that would occur with quadratisation or sparsification. Using simulations to emulate hardware, we predict that a photonic probabilistic computer would outperform the time to solution recently reported for digital annealing units, on the ground state approximation of Erdos-Renyi graph spin-glasses, by orders of magnitude.

==> Contents/EmbeddingSparsification.tex <==
\section{Results on the difficulty of implementing such problems on Ising hardware}
\label{sec:hardware-scaling}

In the previous section we demonstrated how the VCPC is expected to perform, in terms of number of iterations required to reach a particular solution or solution quality. The main argument as to why these problems were chosen is that their geomertries are more amenable to hardware in which connections are implemented virtually.

Here, we demonstrate the growth in the problem sizes considered in the previous sections when employing techniques which would typically be employed in order to fit such problems onto hardware that is not virtually connected or fully connected. This includes, for a higher order problem, quadratisation to turn the energy function into quadratic form, and sparsification or embedding for problems which are quadratic but dense.

\subsection{Set cover problem}
We convert the test instances considered for $k=5$ and $k=10$ to quadratic form, using standard quadratisation procedures, and show the performance between the algorithm on these quadratic energy functions, as compared to directly solving with the heuristic algorithm for the higher order energy function. For both the HUBO and QUBO, we use simulated annealing as the algorithm, since this showed better performance than parallel tempering for the set cover algorithm. 

In Fig.~\ref{subfig:QUBO-HUBO-quality} we plot the performance of the PC-SA algorithm, as previously shown, against a standard annealing solver for QUBO problems. For each, we have the same starting and ending temperature in the cooling schedule, and the same number of iterations in that cooling schedule. The strength parameter, which must necessarily be chosen when quadratising an energy function, was optimised for. As can be seen, while the solution quality for both does not degrade significantly for an increasing number of vertices (note however that the number of iterations linearly scales with increasing hypergraph size, which accounts for the fact that there is no degradation), the solution quality of the QUBO algorithm is worse than that of the HUBO algorithm. Further, increasing the iterations of the QUBO problem did not affect the solution quality.

In Fig.~\ref{subfig:verts_comparison}, we show the growth of the problem size with the quadratisation process for dimension size $k=5$ and $k=10$. This growth for $k=5$ is already quite significant, with the number of QUBO variables corresponding to more than double the number of HUBO variables. For $k=10$, as can be seen in the figure, the slope of this growth increases markedly. In particular, the largest problem sizes of $1000$ vertices for the HUBO problem were converted to, on average, $25000$ vertices for the QUBO. This explains why solution qualities decrease when quadratising, but it is also possible that the quadratisation process makes the enery landscape more difficult to solve, as had been noted in other studies \cite{Dobrynin_2024}.

\begin{figure}
    \centering
    \begin{subfigure}{.45 \linewidth}
        \centering
        \includegraphics[width= \textwidth]{Figures/Main/HS_plot_residual_k=5_QUBO_HUBO.pdf}
        \caption{}
        \label{subfig:QUBO-HUBO-quality}
    \end{subfigure}
    \begin{subfigure}{.45 \linewidth}
        \centering
        \includegraphics[width= \textwidth]{Figures/Main/verts_comparison_plot.pdf}
        \caption{}
        \label{subfig:verts_comparison}
    \end{subfigure}
    \caption{(a) The performance of the PC-SA algorithm, as measured by solution quality, against a standard QUBO SA solver, where the cooling schedules are equivalently parametried (see text). (b) The growth in problem size for randomly generated instances for hypergraph dimensions $k=5$ and $k=10$, when converting the HUBO into a QUBO, a process known as quadratisation.}
    \label{fig:QUBO-HUBO-comparison}
\end{figure}

\subsection{Travelling salesperson problem}
It is known that dense graphs are particularly difficult to embed into hardware. For example, even for efficient embedding algorithms, DWave's $2000$ qubit system only being able to host problems on a complete graph of at most $60$ vertices \cite{Okada_2019}. 

Relatively little is reported on or commented on in the literature related to the geometry of the TSP problem, both without and with $k$-means clustering. Since embeddings or sparsification must be carried out to implement the problem on hardware, understanding this geometry helps to shed light on the difficulty of doing so.


The density of the problem can be seen to scale as
\begin{equation}
    M = \frac{2N^3}{N^4},
\end{equation}
where $N$ is the number of cities (or equivalently, the number of time steps). This follows because each pbit $s_{i,j}$ must be connected to all pbits $s_{i', j'}$ with for any $j$ and with $i'=i$ or $i-1$.
Since $M \rightarrow 0$ as $N \rightarrow \infty$, the problem is not strictly dense, but decays more slowly than any other class of non-dense graphs becuase of the order of the numerator. 

Another property of the geometry which affects embeddability is the size of the largest connected component in the geometry. This is the largest subset of vertices which form a complete graph. This structure is particularly difficult to embed, and places a lower bound on the growth of the problem when the embedding is performed. We find that, for the $52$ city problem with $k$-means clustering, the biggest connected component is of order $100$ vertices. Therefore, both the high number of connections and large connected components we expect would make these difficult problems to find efficient embeddings for, or to sparsify without large growths in problem size.

The usual way to circumvent such embedding difficulties is to break the problem down into subproblems. Although, in principle, one could break down the problem at each step in $k$-means clustering, the geometry of the problem changes at each step due to the mask. This means that the embedding must be calculated $k$ times, and cannot be pre-computed, significantly increasing the complexity of running this on restricted hardware. Similar arguments hold for sparsification: the sparsification procedures must be computed at each step in the $k$-means clustering computation.

We now consider a graph sparsification procedure recently published in Ref.~\cite{Sajeeb_2025}, in the context of solving the TSP. The purpose of graph sparsification is to reduce the density of a problem by enforcing a limit on each p-bit's number of neighbours, at the cost of introducing additional auxiliary p-bits. This connectivity regulation is crucial for non-virtually connected architectures, where large scale fully connected graphs become unfeasible in hardware. The graph sparsification algorithm presented in Ref.~\cite{Sajeeb_2025} achieves sparsification by introducing copy nodes to limit the connectivity to the hyperparameter $k$. Ferromagnetic edges are then introduced between a source node and it's copy nodes in order to correlate their behaviour.

In Fig.~\ref{subfig:sparse-burma14} we show how the number of p-bits for both the unmasked and masked methods varies as the connectivity limit $k$ increases for the burma14 instance. As expected, the KMC masked p-bit array scales more favourably than the unmasked case, as the KMC masked problem is initially denser. It is also worth noting that both cases converge to $\sim 196$ as $k > 51$, as the original unsparsified problems require a connectivity of $\sim 50$. The structure of the VCPC circumvents the hardware issue presented by dense problems, as the number of connections grows linearly with the number of p-bits. In light of this, graph sparsification is unnecessary, enabling us to operate in the unsparsified regime.

\subsection{Spin glasses}
Finally, we consider sparsification of spin glasses. Since we consider Erdős–Rényi random graphs, these are classed as dense graphs with density given by
\begin{equation}
    M = \frac{p N(N-1) }{N(N-1)} = p.
\end{equation}
Thus, for $p=1$, these graphs are as dense as possible and the number of neighbours of every node is equal to $N-1$. There are known results for embedding such graphs into hardware, see for example \cite{Okada_2019}, where using efficient embeddings the size of the embeddable subproblem is around $275$ for $p=0.01$ and $60$ for $p=1$. 

Here, as with the TSP, we focus on sparsification results since these are hardware independent, and allow us to focus on the target number of neighbours as opposed to target architecture. In Fig.~\ref{subfig:sparse-SG} we plot the results for choices of $N=100$ test instances, used in the previous section, for $p=0.1$, $p=0.5$ and $p=1$. As the number of allowed neighbours increases, the number of p-bits in the unsparsified problem is eventually reached. Restricting the number of neighbours to less than $10$, the number of p-bits required to implement a relatively small problem of $100$ p-bits is significant for $p=1$, and approximately above $1000$. This tells us that the problem would grow up to $10$ times to implement on hardware with such constraints. Much hardware does suffer from these constraints, including the Chimera graph structures used by D-Wave, in which each qubit has $6$ neighbours. 

\begin{figure}
    \begin{subfigure}{.49 \linewidth}
\centering
    \includegraphics[width=\textwidth]{Figures/Main/sparse_plot_TSP_v2.pdf}
    \caption{}
    \label{subfig:sparse-burma14}
\end{subfigure}
    \begin{subfigure}{.49 \linewidth}
\centering
\includegraphics[width=\textwidth]{Figures/Main/sparse_plot_SG.pdf}
    \caption{}
    \label{subfig:sparse-SG}
\end{subfigure}
    \caption{The sparsification results for (a) the burma14 instance and (b) an Erdős–Rényi spin glass instance with $N=100$. Plots show the relationship between the number of p-bits and the number of neighours $k$, and for the TSP include results for both masked and unmasked p-bit arrays~\cite{Sajeeb_2025}. }
    \label{fig:sparsification}
\end{figure}


==> Contents/Results.tex <==
\section{Results}
\label{sec:results}
In this section we show how, using simulations, a probabilistic computer would be expected to perform on the three problems of choice. To measure performance, we use a measure called solution quality, $q$, which we define to be the fraction
\begin{equation}
    q = \frac{O_{A}}{O_{\text{ref}}},
\end{equation}
where $O_A$ indicates the best value of the objective function found by the chosen algorithm, whether that be PC-PT or PC-SA, and $O_{\text{ref}}$ refers to the optimal reference objective function. This objective function may be the energy, which will be the case for spin glasses, but could be a different quantity. For the hitting set, for example, it will be the size of the hitting set. The quality $q$ may be larger or smaller than $1$, depending on the choice of objective function, with $1$ being the optimal solution quality. The references will also depend on the choice of algorithm, and since exact numbers are usually not feasible we will use the output of one or a number of other algorithms with documented performance.

\input{Contents/SetCoverResults}
\input{Contents/TSPResults}
\input{Contents/SpinGlassResults}

==> Contents/SetCoverResults.tex <==
\subsection{Set cover}

We now report the results of both simulated annealing and parallel tempering, for set cover, on random instances for a range of sizes of hypergraph. To generate reference hitting set sizes, we use the library \textsc{SetCoverPy} \cite{Zhu2016ANV}, a heuristic algorithm freely available, and which obtains solutions within $1$ percent of the optimal for Beaseley's benchmark set \cite{Beaseley_benchmark}. 

\begin{figure}
    \begin{subfigure}[b]{.5\linewidth}\centering
    \includegraphics[width = \textwidth]{Figures/Main/HUBO_plot_k=5_m=n3.pdf}
    \caption{}
    \label{subfig:soln_k=5}
    \end{subfigure}
    \begin{subfigure}[b]{.5\linewidth}\centering
    \includegraphics[width = \textwidth]{Figures/Main/its_plot_k_10_20_30.pdf}
    \caption{}\label{tab:1a}
    \label{subfig:its-comparison}
    \end{subfigure}\\
    
\begin{subfigure}[b]{.5\linewidth}\centering
    \includegraphics[width = \textwidth]{Figures/Main/scaling_plot_k=5and10_m=n3.pdf}
    \caption{}
    \label{subfig:scaling}
    \end{subfigure}
    \begin{subfigure}[b]{.45\linewidth}\centering
    \includegraphics[width = \textwidth]{Figures/hypergraph_groups_heatmap_n=5000.pdf}
    \caption{}
    \label{subfig:heatmap}
    \end{subfigure}
    \caption{(a) The average solution quality obtained by the PC-PT and PC-SA algorithms for $100$ random hypergraph instances of dimension $k=5$, where the VCPC had $10$ replicas, for an increasing number of vertices. All other parameters are shown in App.~\ref{app:hyperparams}. (b) The solution quality of the PC-SA algorithm for hypergraph dimensions $10$, $20$, $30$ and $40$ with $n=500$ and $m=200$. The error bar shows the range of values obtained for $20$ random instances. (c) The number of iterations required to reach certain solution qualities for hypergraph dimensions $k=5$ and $k=10$, where now a single iteration updates a group of independent p-bits. (d) The variation in the number of independent p-bit groups, $|G|$, versus the hypergraph dimension $k$ and number of hyperedges $m$.}
    \label{fig:HS-results}
\end{figure}
 

Hypergraph dimensions of $k=2$ reduce to QUBO form, so in order to test the performance of the PC-SA and PC-PT algorithms on higher order problems we require that $k>2$. We take $k=5$ for the first tests, but later on show how increasing $k$ changes performance of the algorithm. 

For hypergraphs of dimension $k=5$, we generate $100$ instances for choices of size in the range of $50$ vertices to $1000$ vertices. The results for $k=5$ are shown in Fig.~\ref{subfig:soln_k=5}. The parameters used are listed in App.~\ref{app:hyperparams}. 

Fig.~\ref{subfig:soln_k=5} shows the solution quality, where for this example this is defined as
\begin{equation}
    q = \frac{\text{HS}_{\mathsf{A}}}{\text{HS}_{\mathsf{ref}}},
    \label{eqn:soln-quality}
\end{equation}
and where $text{HS}_{\mathsf{A}}$ refers to the size of the hitting set found by algorithm $A$. Usually, we expect $q\geq 1$ as the algorithm will return a value larger than or equal to that of the reference algorithm, although, $q<1$ is also plausible since the reference size is calculated using a heuristic algorithm, too. As can be seen in the plot, for such dimension of hypergraph, the solution quality for PC-SA was consistenlty higher than $98\%$, which places it as a promising heuristic method for achieving accurate results on hypergraphs with dimension up to $5$ and for vertices up to $1000$. The performance of PC-PT is marginally worse, dropping with increasing hypergraph sizes in contrast to PC-SA. We note, however, that we use linear parallel tempering, which is known to perform worse than adaptive parallel tempering, so future work will aim to clarify the performance of this variant on higher order problems. As part of this it would be interesting to understand in general the performance of parallel tempering algorithms on higher order problems. 

Next, we investigate how the parameter $k$ affects the solution quality for the simulated annealing algorithm. Recall that increasing the dimension of the hypergraph correspond to increasing the order of the energy function to be solved. To investigate this, we plot the solution quality found by the PC-SA algorithm for hypergraphs of size $500$ vertices and $200$ edges, for varying values of $k$ and varying number of iterations. 

For each point we sample $20$ hypergraphs, and run $20$ repeats in parallel \footnote{We avoid calling these replicas, since for the case of parallel tempering replicas refers to the number of chains of different temperatures}. While for $k=10$ we see that the quality approaches $0.95$, for larger values of $k$ the solution quality is worse for an equal number of iterations. This is possibly due to the energy landscape becoming significantly more complex for higher order problems, and therefore more difficult to sample. We leave improvements to this open as a future direction of research.  

In Fig.~\ref{subfig:scaling}, we show how many iterations are needed, on average, to get within a particular solution quality for datasets with $k=5$ and $k=10$. Here, to obtain optimal parallelisation and emphasise the number of iterations needed when such parallelisation can take place, we perform a greedy hypergraph colouring algorithm, which allows us to update multiple independent p-bits at once. As can be seen in the plot, the number of iterations required to reach good solution qualities is significantly reduced from before, where colouring algorithms were not used. For the $k=5$ data, the number of iterations required does not increase significantly in going from finding solutions at $20 \%$ to $10 \%$ larger than the reference algorithm (corresponding to qualities of $1.2$ and $1.1$ respectively) but for $5 \%$ shows a jump in the number of iterations required. This possibly points to the heuristic nature of the simulated annealing algorithm, which can find approximate solutions quickly but struggles more to find more accurate solutions. 

The general trend displayed in the plot is that the number of iterations required to reach a particular solution quality seems to scale reasonably with increasing vertex size. This reduction in required iterations due to the simultaneous update of p-bits in a group is dependent on the number of groups, which is itself dependent on the dimension of the hypergraph considered, as well as the number of hyperedges, when fixing the size of the graph $N$. In Fig.~\ref{subfig:heatmap} we show how this group number changes for $N=5000$. Interesting, for smaller choices of $N$ a similar profile is obtained as shown in App.~\ref{app:heat-plots}. The speedup obtained from group updates is given by the number of vertices divided by the average number of groups, so that a lower number of groups is more optimal. In the worst case, the number of groups is equal to the number of vertices. Thus, for lower hypergraph dimension the best speedups are obtained. On the other hand, for very large dimensions, greedy algorithms perform well, which makes such parameter space less interesting.

As per Eqn.~\ref{eqn:TTS-scaling}, the time to solution requires weighing up the speedup due to parallelisation due to simultaneous p-bit updates and the scaling of $n_{\text{cycles}}({\mathbf{n}})$, or the number of cycles required to complete a single bias update,  with the problem parameters. For a hardware implementation, we find that for a single bias update
\begin{equation}
    n_{\text{cycles}} = 17|E| + C_{\text{misc}} + 256,
\end{equation}
where $C_{\text{misc}}$ is approximately $20$. Since the average group size is $\frac{N}{|G|}$, where $|G|$ is the total number of groups, the time to solution scales as
\begin{equation}
    \text{TTS}_{p, q} = \mathcal{I}_{p,q} \cdot \frac{|G|}{N} \cdot f \cdot \left[ 17|E| + C_{\text{misc}} + 256 \right].
\end{equation}
As such, provided we are in parameter regimes where $|G|$ does not scale as $\mathcal{O}(N)$, and taking $|E|$ to be of order at most $N$, the time to solution depends only on the number of iterations and the clock speed. Since we see that the number of iterations scales linearly with increasing problem size, the VCPC is a promising avenue to solving this higher order problem.






==> Contents/SpinGlassResults.tex <==
\subsection{Spin glasses}
\label{subsec:SG}
\begin{figure}
    \begin{subfigure}{.5 \linewidth}
\centering
    \includegraphics[width=\textwidth]{Figures/Main/ER_plot_all_sizes.pdf}
    \caption{Iteration scaling with density at various sizes}
    \label{subfig:ER-with-p}
\end{subfigure}
    \begin{subfigure}{.5\textwidth}
\centering
\includegraphics[width=\textwidth]{Figures/Main/SA_PT_vs_N_for_p1.pdf}
    \caption{Iteration scaling with graph size at $p=1$}
    \label{subfig:ER-with-N}
\end{subfigure}
    \caption{Showing the number of iterations required to attain solution qualities of $q=0.5,0.8$ over \textbf{(a)} the Erdős–Rényi graph density $p$ and \textbf{(b)} the graph size $N$ at a fixed $p=1$. }
    \label{fig:SG-ER-results}
\end{figure}

Finally, we consider spin glasses on Erdős–Rényi graphs for probabilities ranging from $p=0.1$ to $p=1$. We choose solution qualities of $0.5$ and $0.8$ in order to directly compare to results reported in \cite{Nikhar_2025}, where simulated annealing, parallel tempering, and digital annealing were considered. They showed that the time to solution for digital annealing showed a significant improvement over simulated annealing and parallel tempering algorithms, with time to solutions of graph sizes up to $N=1024$ being below a second for digital annealing, and growing up to of order $10^3$ seconds for parallel tempering.

We therefore consider lattice sizes $N= 100, 250, 500, 750$ and $1024$ and take $q=0.5$ and $q=0.8$, computing the number of iterations required to reach such qualities\footnote{Note that in \cite{Nikhar_2025} they use the terminology `cutoff' rather than solution quality, but the two are equivalent.} shown in Fig.~\ref{subfig:ER-with-p}. We calculate the ground states using large parallel tempering runs (see App.~\ref{app:hyperparams} for the number of iterations and replicas used), which for smaller lattice sizes were chosen based on their consensus of outcomes from the \textsc{MQLib} library of classical algorithms developed for spin-glass ground state calculations \cite{dunning_what_2018}.

Note that for simulated annealing, the number of iterations is the total number $\mathcal{I}$, and in particular we take $I=1$, so that at each $\beta$-step only one iteration is performed. On the other hand, for parallel tempering, the number of replicas is not accounted for in the iteration count. This is because replicas can in theory be replicated in parallel in any hardware implementation. However, since at most $10$ replicas were used in such experiments, even multiplying the number of iterations by the number of replicas would include at most such a factor. 

Based on the number of iterations and placing only moderate assumptions on hardware, we can make estimates from Fig.~\ref{fig:SG-ER-results} about the time to solutions that we expect when running such simulations on dedicated probabilistic hardware. 

==> Contents/TSPResults.tex <==
\subsection{Travelling salesperson problem}

The VCPC's reconfigurable geometry enables us to employ KMC in order to improve the solution quality, where both SA and PT are used sub-methods in the KMC procedure. In both cases, the KMC enhancement greatly reduces the average tour cost and enables convergence nearer to the ground state in the best case scenario. It is also worth noting that we are now able to reduce our penalty weight parameter $A$, while maintaining a high fidelity of valid solutions, as there are fewer states contributing to the possible invalid tours available. We show our hyperparameter choices in Table~\ref{tab:tsp-hparams}.

In Fig.~\ref{fig:tsp-solution-quality} we compare the number of iterations taken to reach various solution qualities for the burma14 instance with the four methods considered. We observe a similar trend in both Fig.~\ref{fig:tsp-solution-quality}a and Fig.~\ref{fig:tsp-solution-quality}b, where PT is able to find lower solutions of a lower quality in several orders of magnitude fewer iterations than SA. This is to be expected, as the lower temperature states are only explored by SA during the latter iterations of the annealing process. The PT algorithm however, is immediately exposed to these lower temperature states, and therefore can explore them constantly. Despite this initial improvement, on average the SA reaches the best solution in less iterations than the PT, both with and without KMC. This is most likely because the simulated annealing schedule evolves $\beta$ smoothly, allowing more consistent convergence toward low-energy states, whereas the rigid temperature exchanges in the 20 replica parallel tempering, can interrupt local relaxation.

% [Harry] results_09 (new colouring)
\begin{table}[htbp]
    \centering
    \caption{Performances on TSPLIB~\cite{Reinelt_1991} benchmark instances using different solvers. Each solver was run 100 times with different seeds, and the results are shown as a fraction of the known optimal solutions. We do not count invalid tours in these averages, where the number of valid tours per method can be seen in the "Valid" columns.}
    \label{tab:tsp-results}

    \renewcommand{\arraystretch}{1.2}
    \begin{tabularx}{\textwidth}{l
        *{6}{>{\centering\arraybackslash}X}
        *{6}{>{\centering\arraybackslash}X}}
        \toprule
        \multirow{2}{*}{\textbf{Instance}} &
        \multicolumn{6}{c}{\textbf{Simulated annealing (SA)}} &
        \multicolumn{6}{c}{\textbf{Parallel tempering (PT)}} \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13}
        & \textbf{Best} & \textbf{Ave.} & \textbf{Valid} & \textbf{Best KMC} & \textbf{Ave. KMC} & \textbf{Valid KMC}
        & \textbf{Best} & \textbf{Ave.} & \textbf{Valid} & \textbf{Best KMC} & \textbf{Ave. KMC} & \textbf{Valid KMC}\\
        \midrule
        burma14     & 1.071  & 1.237  & 100 & 1.000 & 1.079 & 99
                    & 1.089  & 1.222  & 100 & 1.000 & 1.082 & 100 \\
        ulysses16   & 1.169 & 1.303 & 100 & 1.007 & 1.072 & 81
                    & 1.117 & 1.238 & 100 & 1.007 & 1.070 & 83 \\
        ulysses22   & 1.306 & 1.559 & 100 & 1.010 & 1.074 & 91
                    & 1.262 & 1.416 & 100 & 1.010 & 1.072 & 91 \\
        berlin52    & 2.221 & 2.543 & 99 & 1.091 & 1.197 & 99
                    & 2.551 & 2.912 & 42 & 1.049 & 1.199 & 99 \\
        \bottomrule
    \end{tabularx}
\end{table}

In Table~\ref{tab:tsp-results} we show that for smaller instances: burma14, ulysses16 and ulysses22, our results show that KMC enables both SA and PT to converge to within 1$\%$ of the optimal tour for the best case scenario. As well as this the average tour is consistently $\sim7.5\%$ greater than the optimal tour which represents a vast improvement on the standard SA and PT solvers. For the larger instance considered, berlin52, the KMC procedure approximately halves the best and average tour costs for both SA and PT. Remarkably, the fidelity of valid tours is consistently $>80\%$ for every instance and method investigated with the exception of standard PT on berlin52. Despite this, the addition of the KMC procedure in the PT solver enables a best tour cost of 1.049 to be achieved. We show how the distribution of tours obtained changes with the addition of KMC in Fig.~\ref{subfig:berlin52-performance}. As well as this, our scores for berlin52 are comparable to digital annealing results as reported in Ref.~\cite{Ayodele_2022}. Two improvements that could be made would be to utilise the recently published 2D-PT~\cite{Delacour_2025} and Transformer-Augumented-PT~\cite{Bunaiyan_2025} algorithms, to ensure constraint satisfaction and propose pre-learned global moves, respectively.

\begin{figure}
\centering
\begin{subfigure}{.49 \linewidth}
\centering
    \includegraphics[width=\textwidth]{Figures/Main/tsp_solution_quality1.pdf}
    \caption{}
    \label{subfig:sol-quality-tspa}
\end{subfigure}
\begin{subfigure}{.49 \linewidth}
\centering
    \includegraphics[width=\textwidth]{Figures/Main/tsp_solution_quality2.pdf}
    \caption{}
    \label{subfig:sol-quality-tspb}
\end{subfigure}
\caption{The best solution qualities at various numbers of total iterations $\mathcal{I}$ of the SA and PT algorithms without (a) and with (b) KMC. The error bars shows the range of solution qualities obtained for $100$ runs on the burma14 instance.}
    \label{fig:tsp-solution-quality}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.49 \linewidth}
\centering
    \includegraphics[width=\textwidth]{Figures/Main/fig7.pdf}
    \caption{}
    \label{subfig:berlin52-performance}
\end{subfigure}
\caption{Performances of standard SA and $k$-means clustered SA solvers on the berlin52 instance~\cite{Reinelt_1991}, where the optimal tour length is 7542. }
    \label{fig:berlin52_hist_&_sparce_plot}
\end{figure}

\newpage


==> Figures/Main/ER_graph.tex <==

\begin{tikzpicture}[scale = 0.4,
  vertex/.style={circle,draw,fill=green!70,inner sep=2pt},
  edge/.style={}
]

  % ---------- parameters ----------
  \def\N{16}           % number of vertices
  \def\R{4}            % radius of the circle
  \def\pEdge{0.9}     % edge probability (sparser)
  \pgfmathsetseed{2024} % change for a different random graph
  % --------------------------------

  % place vertices around a circle
  \foreach \i in {1,...,\N}{
    \path coordinate (p\i) at ({\R*cos(360*\i/\N)}, {\R*sin(360*\i/\N)});
    \node[vertex] (v\i) at (p\i) {};
  }

  % random edges between distinct pairs
  \foreach \i in {1,...,\N}{
    \pgfmathtruncatemacro{\istart}{\i+1}
    \foreach \j in {\istart,...,\N}{
      \pgfmathsetmacro{\u}{rnd}
      \ifdim \u pt<\pEdge pt
        \draw[edge] (v\i) -- (v\j);
      \fi
    }
  }

\end{tikzpicture}


==> Figures/Main/reconfigurable.tex <==

\begin{tikzpicture}[scale=0.18, vertex/.style={circle,draw,fill=green!70,inner sep=2pt},
  edge/.style={},
  arrow/.style={-{Latex[length=2mm,width=1mm]},thick
                } % shorter arrows
]

% ------- parameters -------
\def\N{12}       % vertices per small graph
\def\r{3}        % radius of each small graph
\def\pEdge{0.4}  % edge probability within each small graph
\def\BigR{10}    % radius of the big ring (spacing between graphs)
% --------------------------

% Macro: one random graph at angle #1, id prefix #2, seed #3
\newcommand{\RandomGraph}[3]{%
  \begin{scope}[shift={(#1:\BigR)}]
    \pgfmathsetseed{#3}%
    % vertices
    \foreach \i in {1,...,\N}{
      \path coordinate (p#2-\i) at ({\r*cos(360*\i/\N)},{\r*sin(360*\i/\N)});
      \node[vertex] (v#2-\i) at (p#2-\i) {};
    }
    % random edges
    \foreach \i in {1,...,\N}{
      \pgfmathtruncatemacro{\istart}{\i+1}
      \foreach \j in {\istart,...,\N}{
        \pgfmathsetmacro{\u}{rnd}
        \ifdim \u pt<\pEdge pt
          \draw[edge] (v#2-\i) -- (v#2-\j);
        \fi
      }
    }
  \end{scope}
}

% Place the four graphs (N, E, S, W)
\RandomGraph{90}{A}{101}   % North
\RandomGraph{0}{B}{202}    % East
\RandomGraph{270}{C}{303}  % South
\RandomGraph{180}{D}{404}  % West

% Curved arrows between them
\draw[arrow,bend left=20] (65:\BigR) to (25:\BigR);
\draw[arrow,bend left=20] (335:\BigR) to (295:\BigR);
\draw[arrow,bend left=20] (245:\BigR) to (205:\BigR);
\draw[arrow,bend left=20] (155:\BigR) to (115:\BigR);

\end{tikzpicture}


==> FileSettings/BibSettings.tex <==
\RequirePackage[biblabel,nomove]{cite} %% add [superscript] option for superscript refs.
\RequirePackage{FileSettings/jabbrv}
\bibliographystyle{FileSettings/naturemag-doi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For bold, numbered bib label
% \makeatletter
% \renewcommand{\@biblabel}[1]{\bfseries\color{color1}#1.}
% \makeatother


==> Tables/table.tex <==
\begin{tabular}{c|ccccc}
          & $V_1$ & $V_2$ & $V_3$ & ... &$V_n$\\
          \hline 
        $0$ & 0 & 1 & 0 & ... & 1\\
        $1$ & 0 & 0 & 1 & ... & 1\\
        $2$ & 1 & 0 & 0 & ... & 0\\
        $3$ & 0 & 1 & 0 & ... & 0\\
        ... & ... & ... & ... & ... & ...\\
        $m$ & 0 & 1 & 0 & ... & 0\\
\end{tabular}

